Adversarial Examples - A Complete Characterisation of the Phenomenon

We provide a complete characterisation of the phenomenon of adversarial examples - inputs intentionally crafted to fool machine learning models. We aim to cover all the important concerns in this field of study: (1) the conjectures on the existence of adversarial examples, (2) the security, safety and robustness implications, (3) the methods used to generate and (4) protect against adversarial examples and (5) the ability of adversarial examples to transfer between different machine learning models. We provide ample background information in an effort to make this document self-contained. Therefore, this document can be used as survey, tutorial or as a catalog of attacks and defences using adversarial examples.

==> chapters/conclusions/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

==> chapters/defences/obfuscate/obfuscate.tex <==
% TODO: talk about transferability between differentiable and non-differentiable models !!!

\subsection{Obfuscated Defences}
\label{subsec:obfuscated_defences}

%\input{chapters/defences/obfuscated}


==> chapters/defences/obfuscated.tex <==
%\subsection{Obfuscated Gradients}
%\cite{athalye2018obfuscated}

%The authors of~\cite{athalye2018obfuscated} identify another reason reason why many defences provide apparent robustn
%Another reason for which defences provide apparent robustness against powerful, iterative, attacks is called \emph{obfuscated gradients}~\cite{athalye2018obfuscated} - a term derived as a special case of gradient masking~\cite{papernot2017practical}.
%Without a good gradient, iterative methods can not follow succeed.
%These phenomena occurs when the gradients are nonexistent or incorrect - caused either intentionally through non-differentiable operations or unintentionally through numerical instability - when the gradient is unstable - due to vanishing/exploding gradients - or randomly due to test-time randomness.


==> chapters/defences/proactive/adversarial_training/training_vs_weight_decay.tex <==
\subsection{Advers}
\label{subsec:training_vs_decay}
% TOOD: label leaking

The first attempt to scale adversarial training to ImageNet~\cite{kurakin2016aadversarial} revealed an interesting phenomena, called 'label leaking' - when a network is trained with adversarial examples, the accuracy on adversarial examples becomes much higher that the accuracy on clean images.
This phenomena triggered the authors of~\cite{galloway2018adversarial} to compare the effects of adversarial training with weight decay - a regularisation technique understood mathematically.
The results suggest that adversarial training can be seen as translating the data \ac{wrt} the loss function, while weight decat scales the let-on-(about-sth/that...)-(to-sb)




==> chapters/defences/proactive/adversarial_training/virtual.tex <==
\subsubsection*{Virtual Adversarial Training}
\label{subsubsec:virtual}

%Towards Safe Deep Learning: Unsupervised Defense Against Generic Adversarial Attacks

==> chapters/defences/proactive/architectures/logit_pairing.tex <==
\subsection{\ac{alp}}
\label{subsuec:logit_pairing}

\ac{alp}~\cite{kannan2018adversarial} is a method that encourages the logits for two images to be similar to each other.
Logit pairing adds a loss penalty $\lambda L(f(\vx), f(\vx')$ for pairs of training examples $\vx$ and $\vx'$, where $\lambda$ is a coefficient that regulates the strength of the penalty and $L$ is a loss function encouraging the logits to be similar.
In practice, the authors use $L^2$ loss.
The method is similar to label smoothing~\cite{szegedy2016rethinking}, a technique showed to offer a small amount of robustness to adversarial examples~\cite{warde201611}.

Logit pairing achieves high accuracy against the attack in Section~\ref{subsec:madry}, considered, at this time, state-of-the art.
Moreover, attacks built on networks trained with \ac{alp} substantially damage black box defences~\cite{tramer2017ensemble}.


==> chapters/defences/proactive/g <==
\subsubsection{\ac{mat}}
\label{subsubsec:multi_strength_training}

Song \etal~\cite{song2017mat} propose a training technique that combines several aplitude of pertubations in the training procedure.
The technique is equivalent to an ensemble of perturbations (Section~\ref{subsec:ensemble}), however training does not happen in a min-max fashion.

Experimental results show improvements in robustness, however, it is not clear if this method is effective when faced with adaptive attacks.



==> chapters/defences/proactive/gans/gradient_adversarial_training.tex <==
\subsubsection{Gradient Adversarial Training}
\label{subsubsec:gradient_adversarial}

Sinha \etal~\cite{sinha2018gradient} propose a new training framework which assumes that simultaneous gradient updates should be statistically indistinguishable from each other.
% TODO: Why? Mention Adversarial
Thus the gradient can be regularised in order to remove salient information that can lead to adversarial examples.
This phenomena, called gradient obfuscation, is described in Section~\ref{}. % TODO: add section on gradient obfuscation
Further on, the gradient tensor is processed in an auxiliary network and then passed to the main network via a gradient reversal procedure.
This training procedure adapts the cross-entropy loss function and adds weight to negative classes whose gradient tensors are similar to those of the primary class.
The weight weight is evaluated using the auxiliary network which indicates the gradient tensors similarities between the primary and negative classes.

Experimental results show better regularisation during training and an increase in robustness when tested against gradient adversarial attacks.
However, robustness is not always preserved when testing is done agaist iterative gradient methods (Section~\ref{subsec:illcm}).



==> chapters/defences/proactive/gans/multi_strength_training.tex <==
\subsubsection{\ac{mat}}
\label{subsubsec:multi_strength_training}

Song \etal~\cite{song2017mat} propose a training technique that combines several aplitude of pertubations in the training procedure.
The technique is equivalent to an ensemble of perturbations (Section~\ref{subsec:ensemble}), however training does not happen in a min-max fashion.

Experimental results show improvements in robustness, however, it is not clear if this method is effective when faced with adaptive attacks.



==> chapters/defences/reactive/detection/detection_efficiency.tex <==
\subsection{On The Overall Efficiency of Detection Methods}
\label{subsubsec:detection_efficiency}


% TODO: review all
\input{chapters/defences/reactive/detection/detection_efficiency}
\input{chapters/defences/reactive/input_transformation/input_transformation_remarks}




An important disadvantage of all the papers presented earlier is their evaluation method.
Because they are tested on simple datasets (such as MNIST~\cite{lecun1998mnist}) or against non adaptive attackers, the results presented in the publications reveal fairly good performance for all detectors.
However, Carlini and Wagner~\cite{carlini2017adversarial} show most detectors perform poorly when faced with an adaptive attacker.
In particular, they use the attack presented in Section~\ref{subsec:carlini} to show that none of the detectors -\cite{bhagoji2018enhancing, feinman2017detecting, gong2017adversarial, grosse2017statistical, hendrycks2016early, metzen2017detecting, li2017adversarial} - are efficient against it.

These results challenge the assumption made at the beginning of this section that adversarial examples have intrinsic differences from natural images.

%% TODO: say neither of those are tested against adaptive attacks!!!

==> chapters/defences/reactive/input_transformation/input_transformation_remarks.tex <==
\subsubsection{Remarks Regarding Input Transformation}
% They do not generalise, so one input transformation should be applied to a specific architecture, which makes such techniques hard to apply
